Mixed Strategy Game Model Against Data Poisoning Attacks

In this paper we use game theory to model poisoning attack scenarios. We prove the non-existence of pure strategy Nash Equilibrium in the attacker and defender game. We then propose a mixed extension of our game model and an algorithm to approximate the Nash Equilibrium strategy for the defender. We then demonstrate the effectiveness of the mixed defence strategy generated by the algorithm, in an experiment.

==> Sections/pure_strategy.tex <==

 \section{Finding Pure NE: Saddle Points}
 
 
 \textcolor{red}{The $\theta$ side is not differentiable, therefore this method is impossible to use}
 To find the saddle points in $O_A$, we need to solve for $D_C$ and $\theta$ in the following system:
 \begin{equation}
    \nabla_{D_c} O_A (D_{val},D_C,\theta) = \nabla_{\theta} O_A(D_{val},D_C,\theta)= 0
    \end{equation}
    \begin{equation}
    \nabla_{D_c}\nabla_{D_c} O_A * \nabla_{\theta}\nabla_{\theta} O_A - ( \nabla_{D_c}\nabla_{\theta} O_A )^2 < 0
    \end{equation}
    \begin{equation}
        0<=\theta<=1
    \end{equation}
Any $\theta$ and feasible $D_C$ pair satisfying the equations above corresponds to a pure NE strategy set for the attacker and the defender. The accuracy impact to the ML algorithm will be the value of $O_A (D_{val},D_C,\theta)$.
 
